Automated Trustworthiness Oracle Generation for Machine Learning Text Classifiers

Machine learning (ML) for text classification has been widely used in various domains. These applications can significantly impact ethics, economics, and human behavior, raising serious concerns about trusting ML decisions. Studies indicate that conventional metrics are insufficient to build human trust in ML models. These models often learn spurious correlations and predict based on them. In the real world, their performance can deteriorate significantly. To avoid this, a common practice is to test whether predictions are reasonable based on valid patterns in the data. Along with this, a challenge known as the trustworthiness oracle problem has been introduced. Due to the lack of automated trustworthiness oracles, the assessment requires manual validation of the decision process disclosed by explanation methods. However, this is time-consuming, error-prone, and unscalable. We propose TOKI, the first automated trustworthiness oracle generation method for text classifiers. TOKI automatically checks whether the words contributing the most to a prediction are semantically related to the predicted class. Specifically, we leverage ML explanations to extract the decision-contributing words and measure their semantic relatedness with the class based on word embeddings. We also introduce a novel adversarial attack method that targets trustworthiness vulnerabilities identified by TOKI. To evaluate their alignment with human judgement, experiments are conducted. We compare TOKI with a naive baseline based solely on model confidence and TOKI-guided adversarial attack method with A2T, a SOTA adversarial attack method. Results show that relying on prediction uncertainty cannot effectively distinguish between trustworthy and untrustworthy predictions, TOKI achieves 142% higher accuracy than the naive baseline, and TOKI-guided attack method is more effective with fewer perturbations than A2T.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut samples/*.toc \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.12   Bug fixes
	       Switched to unicode-math and libertinus for Unicode engines

Version 2.11   Conference date is no longer printed in bibstrip.
	       ISBN now uses 4-digit year
	       DOI in bibliography is now output as doi:XX.XXXX/XXXXX.XXXX
	       Changed URL in Creative Commons licenses (deleted
	       trailing /legalcode)

Version 2.10.  Bug fixes.  Documentation update.

Version 2.09.  Experimental tagging code is now in the main branch.
	       Creative Commons license is now allowed for all materials. 

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> sections/background.tex <==
% \valerio{I suggest to add a section "Problem Definition" where we explain what we want to do, I found it very useful when papers like ours have a goal that is relatively new. It would be good for us, as in a "Problem Definition" section we can clarify what we mean by trustworthiness (currently the definition is buried in the text) and what we want to achieve. }

% \valerio{Usually, it should be avoided to just list and explain the "background" without any context. It should be more clear why readers have to know this background and how this relates to our technique}
\lam{I added a paragraph at the beginning of "background" as well as concluded the usage of listed techniques at the end of each subsection to explain why readers have to know this background and how this relates to our technique.}

Two major challenges arise when addressing the trustworthiness oracle problem presented in Problem~\ref{prob:trustworthiness_oracle}.
Firstly, most text classifiers are black-box, making it difficult to uncover the reasoning behind their predictions.
Secondly, after explaining the prediction, a measurement of semantic relatedness between words in the explanation and the predicted class is required. 
This section outlines several state-of-the-art techniques that can address these two challenges. 

\lam{I plan to summarise this section to reduce the length of the paper.}

\valerio{Yes, Section 3 is too long the reader should start to read the technique after section 2, can we just make this backgorund shorter an un put inside the methodlogy when we discuss explainability and word embedding. also, a couple of sentences explaining how LIME works would be useful in Section I or Section II.  }
\subsection{Explainability for ML} 
\label{sec:explainability}

% \valerio{Since we are using Lime we should explain how lime works here. Also, not sure why we are focusing too much on LLMs, this things are general to any black box models.}
% \lam{Revised it to explain how lime works and made this subsection more general for ML models.}
% LLMs are primarily complex ``black-box'' systems, presenting significant challenges for model interpretation. 
The black-box property of ML, especially text classifiers, presents significant challenges for model interpretation.
This lack of model interpretation can lead to misclassification or hallucinations in some cases~\cite{Weidinger:2022:TaxonomyofRisksposedbyLanguageModels}. 
% Therefore, it is critical to develop explainability to understand how these powerful models work.
Various explanation methods have been proposed to develop explainability for ML models, which are typically divided into two main categories: \textit{global} and \textit{local} explanations.

Global explanations provide insights into the inner workings of the entire model, following the reasoning leading to all possible outcomes. 
They aim to understand what individual components have encoded and explain the knowledge properties learned by these components~\cite{Zhao:2024:ExplainabilityforLargeLanguageModelsASurvey}.
Probing methods are commonly applied in various studies~\cite{Tenney:2018:WhatDoYouLearnFromContextProbingForSentenceStructureInContextualizedWordRepresentations, Sorodoc:2020:ProbingforReferentialInformationinLanguageModels, Clark:2019:WhatDoesBERTLookatAnAnalysisofBERTsAttention, Kovaleva:2019:RevealingtheDarkSecretsofBERT, Wu:2020:StructuredSelfAttentionWeightsEncodeSemanticsinSentimentAnalysis, Marvin:2018:TargetedSyntacticEvaluationofLanguageModels, Ravichander:2020:OntheSystematicityofProbingContextualizedWordRepresentationsTheCaseofHypernymyinBERT} to analyse model representations and parameters, thereby understanding the knowledge captured by ML models.
Alternatively, several studies~\cite{Bau:2018:IdentifyingandControllingImportantNeuronsinNeuralMachineTranslation, Dalvi:2019:WhatIsOneGrainofSandintheDesert?AnalyzingIndividualNeuronsinDeepNLPModels, Torroba:2020:IntrinsicProbingthroughDimensionSelection, Openai:2024:GPT4TechnicalReport, Singh:2023:ExplainingBlackBoxTextModulesInNaturalLanguageWithLanguageModels} 
% , instead of examining the whole vector space, 
analyse neuron activation to determine model responsiveness to input.
Others~\cite{Kim:2018:InterpretabilityBeyondFeatureAttributionQuantitativeTestingwithConceptActivationVectorsTCAV} map inputs to a set of concepts and measure the importance of each concept to model predictions.
% Recent works~\cite{Kim:2018:InterpretabilityBeyondFeatureAttributionQuantitativeTestingwithConceptActivationVectorsTCAV} also focus on concept-based methods to understand models’ knowledge.
Recently, mechanistic interpretation~\cite{Bricken:2023:TowardsMonosemanticity:DecomposingLanguageModelsWithDictionaryLearning, Geva:2021:TransformerFeedForwardLayersAreKeyValueMemories, Meng:2022:LocatingandEditingFactualAssociationsinGPT, Geva:2022:TransformerFeedForwardLayersBuildPredictionsbyPromotingConceptsintheVocabularySpace, Lieberum:2023:DoesCircuitAnalysisInterpretabilityScaleEvidencefromMultipleChoiceCapabilitiesinChinchilla} is applied to understand ML models by investigating individual neurons and especially their connections.
Although a multitude of techniques~\cite{Caruana:2015:IntelligibleModelsforHealthCarePredictingPneumoniaRiskandHospital30dayReadmission, Benjamin:2015:InterpretableClassifiersUsingRulesAndBayesianAnalysis:BuildingABetterStrokePredictionModel, Yang:2018:GlobalModelInterpretationViaRecursivePartitioning, Zupon:2019:LightlysupervisedRepresentationLearningwithGlobalInterpretability, Anh:2016:SynthesizingThePreferredInputsForNeuronsInNeuralNetworksViaDeepGeneratorNetworks} are proposed to enable global explanations, they are challenging to achieve in practice, especially for models with a large number of parameters~\cite{Adadi:2018:PeekingInsidetheBlackBoxASurveyonExplainableArtificialIntelligenceXAI}. 

Different from global explanations, local explanations focus on individual predictions
% generated by LLMs
for a specific input.
There is a wide range of different approaches that enable local explanations~\cite{Zhao:2024:ExplainabilityforLargeLanguageModelsASurvey}.
% feature attribution
The first approach, feature attribution, aims to measure the relevance of each input feature, such as a word, to a prediction.
The attributions of individual words can be measured in various ways.
Several methods, such as LIME~\cite{Ribeiro:2016:WhyShouldITrustYouExplainingthePredictionsofAnyClassifier}, locally approximate the original model as an interpretable surrogate model by randomly sampling neighbors around the input~\cite{Ribeiro:2016:WhyShouldITrustYouExplainingthePredictionsofAnyClassifier, Ribeiro:2018:Anchors:HighPrecisionModelAgnosticExplanations, Lundberg:2017:AUnifiedApproachtoInterpretingModelPredictions}.
Other methods~\cite{Robnik:2008:ExplainingClassificationsForIndividualInstances, David:2014:ExplainingDataDrivenDocumentClassifications, Li:2016:VisualizingandUnderstandingNeuralModelsinNLP, Fong:2017:InterpretableExplanationsofBlackBoxesbyMeaningfulPerturbation, Li:2017:UnderstandingNeuralNetworksthroughRepresentationErasure, Kádár:2017:RepresentationofLinguisticFormandFunctioninRecurrentNeuralNetworks, Jing:2018:DistributionFreePredictiveInferenceforRegression, Wu:2020:PerturbedMaskingParameterfreeProbingforAnalyzingandInterpretingBERT} perturb input
% ,  such as removing, masking, or altering words,
and evaluate model output changes.
Some methods~\cite{Simonyan:2014:DeepInsideConvolutionalNetworksVisualisingImageClassificationModelsandSaliencyMaps, Aubakirova:2016:InterpretingNeuralNetworkstoImprovePolitenessComprehension, Andrew:2017:RightfortheRightReasonsTrainingDifferentiableModelsbyConstrainingtheirExplanations, Sundararajan:2017:AxiomaticAttributionforDeepNetworks, Kindermans:2019:TheUnreliabilityofSaliencyMethods, Mohebbi:2021:ExploringtheRoleofBERTTokenRepresentationstoExplainSentenceProbingResults} compute the gradient of the output with respect to the input.
Another way to measure word attributions is through decomposition~\cite{Grégoire:2017:ExplainingNonlinearClassificationDecisionsWithDeepTaylorDecomposition, Bach:2016:ControllingExplanatoryHeatmapResolutionAndSemanticsViaDecompositionDepth}.
% attention mechanism
The second approach, attention mechanism, captures meaningful correlations between intermediate states of input to explain the predictions.
Attention-based explanations are categorised into two main groups: visualisation methods~\cite{Vig:2019:AMultiscaleVisualizationofAttentionintheTransformerModel, Jaunet:2022:VisQA:XrayingVisionandLanguageReasoninginTransformers, Hoover:2020:exBERT:AVisualAnalysisTooltoExploreLearnedRepresentationsinTransformerModels, Park:2019:SANVis:VisualAnalyticsforUnderstandingSelfAttentionNetworks, Yeh:2024:AttentionViz:AGlobalViewofTransformerAttention, DeRose:2021:AttentionFlowsAnalyzingandComparingAttentionMechanismsinLanguageModels} and function-based methods~\cite{Barkan:2021:GradSAM:ExplainingTransformersviaGradientSelfAttentionMaps, Hao:2021:SelfAttentionAttribution:InterpretingInformationInteractionsInsideTransformer}.
However, there is an extensive debate in research on whether attention weights are suitable for explanations, and the validity of this approach is unlikely to be resolved soon~\cite{Jain:2019:AttentionisnotExplanation, Serrano:2019:IsAttentionInterpretable, Mohankumar:2020:TowardsTransparentandExplainableAttentionModels}.
The third approach explains model behavior from the perspective of individual instances, illustrating how the model output changes with different inputs~\cite{Koh:2017:UnderstandingBlack-boxPredictionsviaInfluenceFunctions, Jin:2020:IsBERTReallyRobustAStrongBaselineforNaturalLanguageAttackonTextClassificationandEntailment, Garg:2020:BAE:BERTbasedAdversarialExamplesforTextClassification, Li:2021:ContextualizedPerturbationforTextualAdversarialAttack, Wang:2022:SemAttack:NaturalTextualAttacksviaDifferentSemanticSpaces, Wu:2021:Polyjuice:GeneratingCounterfactualsforExplainingEvaluatingandImprovingModels, Ross:2021:ExplainingNLPModelsviaMinimalContrastiveEditingMiCE, Treviso:2023:CREST:AJointFrameworkforRationalizationandCounterfactualTextGeneration}.
The last approach generates texts in natural languages to explain a prediction~\cite{Rajani:2019:ExplainYourselfLeveragingLanguageModelsforCommonsenseReasoning, Liu:2019:TowardsExplainableNLPAGenerativeExplanationFrameworkforTextClassification}.
However, the reliability of applying these natural language explanations still necessitates further investigation.

To address the trustworthiness oracle problem, this paper applies local explanation methods that follow the feature attribution approach to uncover the reasoning behind model predictions. 
There are two primary reasons justifying this choice. 
Firstly, analogously to humans, who focus on understanding only part of a model to comprehend the whole, local explanations are more readily applicable.
Secondly, while other local explanation approaches are subject to extensive debate, methods following the feature attribution approach, such as the state-of-the-art LIME~\cite{Ribeiro:2016:WhyShouldITrustYouExplainingthePredictionsofAnyClassifier}, SHAP~\cite{Lundberg:2017:AUnifiedApproachtoInterpretingModelPredictions}, and IG~\cite{Sundararajan:2017:AxiomaticAttributionforDeepNetworks}, have been demonstrated their effectiveness and widely used by AI practitioners.


\subsection{Word Embedding}

Word embedding methods are widely used in Natural Language Processing (NLP) to measure the semantic similarity between words. 
They provide fixed-length vector representations of words, capturing their internal semantic and syntactic information.
The concept of word embedding was first introduced with Neural Networks Language Model (NNLM)~\cite{Bengio:2000:ANeuralProbabilisticLanguageModel, Bengio:2001:ExperimentsOnTheApplicationOfIohmmsToModelFinancialReturnsSeries}.
The motivation behind this is that words are more likely to share similar meanings if they are in the same context~\cite{Harris:1954:DistributionalStructure}.
Their idea is to reframe the problem as an unsupervised learning problem, with the projection of raw word vectors into an embedding layer before being fed into other layers of the network.
Word embeddings have since become a topic that attracts attention from both the research community and the industry. They are not only used as standalone features in many NLP tasks~\cite{Turian:2010:WordRepresentations:ASimpleAndGeneralMethodForSemisupervisedLearning} but they also encode accurate syntactic and semantic word relationships~\cite{Mikolov:2013:LinguisticRegularitiesinContinuousSpaceWordRepresentations}. 

Nowadays, the existing word embedding methods are diverse, leveraging both local and global information.
Several methods focus on word’s contexts, such as the continuous bag-of-words (CBOW) and skip-gram (SG) models~\cite{Mikolov:2013:EfficientEstimationofWordRepresentationsinVectorSpace, Mikolov:2013:DistributedRepresentationsofWordsandPhrasesandtheirCompositionality}.
While CBOW trains a model to predict the centre word based on its context, SG reverses the roles, where the centre word is used to predict each word appearing in its context. 
FastText~\cite{Bojanowski:2017:FastText:EnrichingWordVectorswithSubwordInformation, Joulin:2017:BagofTricksforEfficientTextClassification} is a well-known improvement over the SG model, particularly effective for embedding rare words.
Other methods, on the other hand, use global information, generally corpus-wide statistics such as word-context co-occurrence counts.
For example, GloVe~\cite{Pennington:2014:Glove:GlobalVectorsforWordRepresentation} trains a log-linear model to encode semantic relationships between words as vector offsets in the learned vector space, using co-occurrence ratios rather than raw counts.
Recently, a new model for deep contextualised word representation, Embeddings from Language Models (ELMo)~\cite{Peters:2018:DeepContextualizedWordRepresentations}, was introduced to effectively capture complex word characteristics and usage across different linguistic contexts. 
An ELMo representation is generated by considering an entire sentence as the input.
% Specifically, the function is generated by a bidirectional LSTM network trained with a coupled language model. 
By incorporating the ELMo representation, existing embedding models can be improved by capturing the sentence information. 
ELMo also leads to the development of a series of pre-trained neural network models for language tasks, such as BERT~\cite{Devlin::2019:BERTPretrainingofDeepBidirectionalTransformersforLanguageUnderstanding} and OpenAI GPT~\cite{Radford:2018:ImprovingLanguageUnderstandingByGenerativePretraining}. Their effectiveness is demonstrated across a range of language tasks~\cite{Wang:2019:EvaluatingWordEmbeddingModelsMethodsAndExperimentalResults}.

In this paper, word embedding methods are used to evaluate how semantically related words in the explanation are to the class.
\lam{Explain why we use multiples word embedding models}
However, word embedding themselves can be prone to biases due to their training data~\cite{Bolukbasi:2016:ManistoComputerProgrammerasWomanistoHomemakerDebiasingWordEmbeddings, Wang:2019:EvaluatingWordEmbeddingModelsMethodsAndExperimentalResults, Torregrossa:2021:ASurveyOnTrainingAndEvaluationOfWordEmbeddings, Schuster:2020:HumptyDumpty:ControllingWordMeaningsviaCorpusPoisoning}, which potentially impacts the ability to measure the semantic relatedness between words.
To mitigate this, we apply ensemble learning~\cite{Polikar:2012:EnsembleLearning, Dong:2020:ASurveyonEnsembleLearning, Kumar:2022:AComprehensiveSurveyonEnsembleMethods} by employing different word embedding methods. 

% \subsection{Trustworthiness of LLMs}

% AI practitioners, including researchers, developers, and decision-makers traditionally evaluate ML models, including LLMs, based on various properties.
% Specifically, system performance, such as accuracy, typically serves as the primary criterion in many workflows. 
% However, relying solely on this metric is insufficient to ensure the model's quality and trustworthiness. 
% If a model lacks trustworthiness, it is unlikely to be deployed in the real world.
% Trustworthiness is a complex concept that has raised numerous scholarly debates among researchers across diverse disciplines. 
% It can be defined by many as the combination of a variety of concepts, such as robustness, security, transparency, fairness, and safety~\cite{Wing:2021:TrustworthyAI, Thiebes:2021:TrustworthyArtificialIntelligence, Liu:2022:TrustworthyAIAComputationalPerspective, Kaur:2022:TrustworthyArtificialIntelligenceAReview, Li:2023:TrustworthyAIFromPrinciplestoPractices}.
% However, this definition is neither clear nor complete and does not fully capture the essence of the concept. 
% Therefore, this paper adopts the definition of trustworthiness proposed by Kästner et al.~\cite{Kästner:2021:OntheRelationofTrustandExplainabilityWhytoEngineerforTrustworthiness}: 
% \textit{a system is trustworthy to a stakeholder in a given context if and only if it works properly in the context and the stakeholder has justified belief in it.}
% \valerio{Steven and I used an almost identical definition but with a different citation (see Steven's thesis), please double check we are citing the correct source :) }
% \steven{Source seems like it's the correct one}
% % Kästner et al. also distinguish between trust and trustworthiness, where trust is the perception a person has towards a system, while trustworthiness is a property of that system. 
% % People can trust an untrustworthy system, and vice versa.
% Following this definition, if we want to be justified in our beliefs about how well a system works, it often is helpful to have a sufficient understanding of the system. 
% Convincing explanations can help us to gain this understanding and justification. 
% Therefore, it is a common sentiment that model explanations can promote trustworthiness~\cite{Kästner:2021:OntheRelationofTrustandExplainabilityWhytoEngineerforTrustworthiness, Lipton:2018:TheMythosOfModelInterpretabilityInMachineLearningTheConceptOfInterpretabilityIsBothImportantAndSlippery}.
% One of the key properties of explanations is \textit{plausibility}, referring to how convincing the explanation is to a human~\cite{Wiegreffe:2019:AttentionIsNotNotExplanation}.
% In the context of LLMs, a trustworthy LLM should be able to explain its reasoning 
% % and provide transparency 
% regarding its decision-making process~\cite{Liu:2023:TrustworthyLLMsaSurveyandGuidelineforEvaluatingLargeLanguageModelsAlignment} that matches human rationales.
% \steven{If you're deciding to use the term 'rationale' then you should probably define it (it's been used in several different ways before).}
% % such as by highlighting relevant words or phrases in the texts.
% However, whether current LLMs truly reason logically in a human-like manner remains debatable. There is mounting evidence suggesting that LLMs can provide seemingly sensible but ultimately incorrect or invalid justifications~\cite{Turpin:2023:LanguageModelsDontAlwaysSayWhatTheyThinkUnfaithfulExplanationsinChainofThoughtPrompting, Frieder:2023:MathematicalCapabilitiesofChatGPT}. 
% Furthermore, LLMs are known to exploit superficial spurious correlations in the training data rather than meaningful logic~\cite{Du::2021:TowardsInterpretingandMitigatingShortcutLearningBehaviorofNLUmodels}.
% % This paper focuses on the evaluation of the trustworthiness of an LLM through the proxy of the plausibility of its explanations.
% In order to address the above challenges, we propose two different approaches for generating fully automated oracles that can assess the trustworthiness of predictions made by any LLMs.
% In this paper, the \textit{plausibility} of explanations also acts as the proxy for evaluating the trustworthiness of predictions made by LLMs.

==> sections/motivating_example.tex <==
% \lam{I revised this subsection to make it clearer}
% \begin{figure*}[ht]
%     \centering
%     \begin{subfigure}[ht]{0.48\linewidth}
%         \centering
%         \includegraphics[width=1\linewidth, trim={0 14.4cm 0 0}, clip]{figures/20news_example.pdf}
%         \caption{Prediction determining if a document is about Christianity or Atheism}
%     \end{subfigure}%
%     \hfill
%     \begin{subfigure}[ht]{0.48\linewidth}
%         \centering
%         \includegraphics[width=1\linewidth, trim={0 14.8cm 0 0}, clip]{figures/amazon_example.pdf}
%         \caption{Prediction analysing amazon review polarity}
%     \end{subfigure}
%     \caption{LIME explanations of individual predictions with strong confidences. The color indicates which class the word contributes to. The shade represents the importance given to the most relevant words highlighted in the text.}
%     \label{fig:motivating_example}
% \end{figure*}

% \valerio{This is the first time you mentioned lime, is our of the blue we should mention it earlier in the introduction}
% \neelofar{it can be added in section~\ref{sec:explainability}}
% \lam{I mentioned LIME in the introduction and also describe LIME in section~\ref{sec:explainability}}
% ML models might make confident predictions but rely on spurious patterns, 
ML models might learn spurious correlations in the training data and overconfidently predict based on them,
leading to problematic predictions in the real world.
For example,
Figures~\ref{fig:20news_example} and~\ref{fig:amazon_example} show two text inputs: one for a binary classification task on Christianity and Atheism using a feedforward neural network~\cite{Dong:2018:ComparingAutomaticandHumanEvaluationofLocalExplanationsforTextClassification}, and the other for a binary sentiment classification task using a fine-tuned model\footnote{https://huggingface.co/pig4431/amazonPolarity\_roBERTa\_5E}.
Each figure also shows the model's prediction and its LIME explanation~\cite{Ribeiro:2016:WhyShouldITrustYouExplainingthePredictionsofAnyClassifier}. 
\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.495\linewidth}
        \centering
        \includegraphics[width=1.\linewidth, trim={0 25.3cm 0 3mm}, clip]{figures/amazon_example_ori.pdf}
        \vspace{-6.3mm}
        \caption{Original text}
        \label{fig:amazon_example}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.495\linewidth}
        \centering
        \includegraphics[width=1.\linewidth, trim={0 25.3cm 0 3mm}, clip]{figures/amazon_example_rem.pdf}
        \vspace{-6.3mm}
        \caption{Irrelevant words removed}
        \label{fig:amazon_remove_words}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.495\linewidth}
        \centering
        \includegraphics[width=1.\linewidth, trim={0 24.8cm 0 -5mm}, clip]{figures/amazon_example_tricked_or.pdf}
        \caption{A trustworthy prediction of a positive review}
        \label{fig:original_trust_prediction}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.495\linewidth}
        \centering
        \includegraphics[width=1.\linewidth, trim={0 24.8cm 0 -5mm}, clip]{figures/amazon_example_tricked.pdf}
        % \llap{\raisebox{2cm}{%  move next graphics to top right corner
        %     \includegraphics[width=1.\linewidth, trim={0 28.6cm 10cm 0}, clip]{figures/amazon_example_tricked_or.pdf}%
        % }}
        \caption{The same review with irrelevant words injected}
        \label{fig:falied_synthesised_data}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[ht]{0.495\linewidth}
        \centering
        \includegraphics[width=1.\linewidth, trim={0 25.3cm 0 -5mm}, clip]{figures/amazon_example_attack.pdf}
        \caption{An adversarial example generated by TextAttack}
        \label{fig:bae_adversarial_attack}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[ht]{0.49\linewidth}
        \centering
        \includegraphics[width=1.\linewidth, trim={0 25.3cm 0 -5mm}, clip]{figures/amazon_example_man_attack.pdf}
        \caption{An adversarial example generated manually}
        \label{fig:man_adversarial_attack}
    \end{subfigure}%
    \caption{LIME explanations of predictions analysing amazon reviews.
    % The color indicates which class the word contributes to. The shade represents the importance given to the words highlighted in the text.
    Words highlighted in \textcolor{myorange}{orange} and \textcolor{myblue}{blue} indicate which class, \textcolor{myorange}{\textbf{negative}} or \textcolor{myblue}{\textbf{positive}}, they contribute to, with the shade representing their importance.
    }
    \Description[Examples for differentiating trustworthiness and robustness]{Fully described in the text.}
\end{figure}
% Figures~\ref{fig:20news_example} and~\ref{fig:amazon_example} illustrate LIME explanations~\cite{Ribeiro:2016:WhyShouldITrustYouExplainingthePredictionsofAnyClassifier} for two individual predictions. 
% % \begin{figure}[ht]
% %     \centering
% %     \includegraphics[width=1\linewidth, trim={0 14.8cm 0 0}, clip]{figures/amazon_example.pdf}
% %     \caption{LIME explanation of a prediction analysing amazon review polarity. The color indicates which class the word contributes to. The shade represents the importance given to the most relevant words highlighted in the text.}
% %     \label{fig:amazon_example}
% %     \Description[The prediction is based on words that do not reflect sentiment meanings]{Fully described in the text.}
% % \end{figure}
% % \begin{figure}[ht]
% %     \centering
% %     \begin{subfigure}[ht]{1\linewidth}
% %         \centering
% %         \includegraphics[width=1\linewidth, trim={0 14.8cm 0 0}, clip]{figures/amazon_example.pdf}
% %         \caption{Prediction of the original data}
% %         \label{fig:amazon_example}
% %     \end{subfigure}%
% %     \hfill
% %     \begin{subfigure}[ht]{1\linewidth}
% %         \centering
% %         \includegraphics[width=1\linewidth, trim={0 14.4cm 0 0}, clip]{figures/test_bae.pdf}
% %         \caption{Prediction of an adversarial example generated by TextAttack}
% %         \label{fig:bae_adversarial_attack}
% %     \end{subfigure}%
% %     \hfill
% %     \begin{subfigure}[ht]{1\linewidth}
% %         \centering
% %         \includegraphics[width=1\linewidth, trim={0 16.8cm 0 0}, clip]{figures/test-fail-new.pdf}
% %         \caption{Prediction of manually synthesised data}
% %         \label{fig:falied_synthesised_data}
% %     \end{subfigure}
% %     \caption{LIME explanation of predictions analysing amazon review polarity. 
% %     % The color indicates which class the word contributes to. The shade represents the importance given to the most relevant words highlighted in the text.
% %     }
% %     \Description[Examples for differentiating trustworthiness and robustness]{Fully described in the text.}
% % \end{figure}
% The first prediction is made by a feedforward neural network~\cite{Dong:2018:ComparingAutomaticandHumanEvaluationofLocalExplanationsforTextClassification} trying to determine if a document is about Christianity or Atheism. %, with 0.939 accuracy.
% The second prediction is generated by a fine-tuned model
% % \footnote{https://huggingface.co/pig4431/amazonPolarity\_roBERTa\_5E}
% analysing amazon review polarity. % which achieves an accuracy of 0.933.
Although both predictions are correct with strong confidences of 0.995 and 0.999,
% The first model classifies that the document is about Atheism, while the second one analyses the review as negative.
% However, 
their explanations reveal their arbitrary reasoning. 
In the first explanation, the most relevant words ``Nntp'' and ``Host'' are semantically related to neither class but appear frequently in the Atheism examples~\cite{Ribeiro:2016:WhyShouldITrustYouExplainingthePredictionsofAnyClassifier}. 
% These words appear in 22\% of the training examples, 99\% of them in the class Atheism~\cite{Ribeiro:2016:WhyShouldITrustYouExplainingthePredictionsofAnyClassifier}. 
% Even if headers are removed, the model still selects proper names and email addresses of prolific posters from the original newsgroups~\cite{Ribeiro:2016:WhyShouldITrustYouExplainingthePredictionsofAnyClassifier}.
In the second explanation, 
% most highlighted words are semantically unrelated to both classes. T
the most relevant word ``BUT'' is a functional word while other relevant words ``idea'', ``It'', ``the'', etc., do not reflect the sentiment polarity. 
% Moreover, the word ``hype'' seems more semantically related to positive sentiment, despite the predicted class being negative.
Examining these explanations suggests the predictions are untrustworthy as they are not made for the right and meaningful reasons.

Figures~\ref{fig:20news_example_rem} and~\ref{fig:amazon_remove_words} demonstrate the impact of removing irrelevant words from the inputs.
In Figure~\ref{fig:20news_example_rem}, the document is now misclassified as Christianity by the same model.
In Figure~\ref{fig:amazon_remove_words}, despite negative sentiment in phrases ``not seen him CLEAN'', ``slow'', ``rough patch'', and ``sloggin'', the model fails to predict correctly without the spurious correlations.
To further test the potential harm of the untrustworthy prediction in Figure~\ref{fig:amazon_example}, we synthesise a new text input from a positive review shown in Figure~\ref{fig:original_trust_prediction} by injecting the orange-highlighted words ``back'', ``not'', and ``BUT''.
The original text is correctly predicted with a high confidence of 0.990 and the injected words do not change the original meaning.
However, the new prediction, as shown in Figure~\ref{fig:falied_synthesised_data} with the injected words underlined, is incorrect.
The model misinterprets the injected words as clues for a negative review, showing that it is misled by minor spurious correlations.
These examples underscore the importance of trustworthiness testing.
If trustworthiness issues are not detected early, ML models might misclassify real-world data without spurious correlations or be fooled by spurious correlations, leading to problematic predictions.

% Although the models achieve held-out accuracies of 0.939 and 0.933, respectively, they do not generalise and are likely to fail in the real world. 
% Manual examining the reasoning behind predictions through explanations is a way to address the trustworthiness oracle problem. 
% However, this process is not only time-consuming but also prone to human bias, especially when dealing with large datasets. 


We differentiate trustworthiness from robustness by revisiting the prediction in Figure~\ref{fig:amazon_example}, showing that robustness testing is unable to identify issues in the model's behavior, but trustworthiness testing can.
TextAttack,
% \footnote{https://github.com/QData/TextAttack}, 
a framework implementing several state-of-the-art adversarial example generation methods~\cite{Morris:2020:TextAttack:AFrameworkforAdversarialAttacksDataAugmentationandAdversarialTraininginNLP}, is applied to attack~\cite{Zhang:2020:AdversarialAttacksonDeeplearningModelsinNaturalLanguageProcessingASurvey} the model on the same text input.
% BAE~\cite{Garg:2020:BAE:BERTbasedAdversarialExamplesforTextClassification}, an adversarial example generation implemented in TextAttack\footnote{https://github.com/QData/TextAttack}~\cite{Morris:2020:TextAttack:AFrameworkforAdversarialAttacksDataAugmentationandAdversarialTraininginNLP}, is applied to adversarial attack~\cite{Yuan:2019:AdversarialExamplesAttacksandDefensesforDeepLearning} the given model on the same text input.
An additional adversarial example is generated manually to ensure grammar and semantic preservation by replacing orange-highlighted words in Figure~\ref{fig:amazon_example} with their synonyms from WordNet~\cite{Miller:1995:WordNetALexicalDatabaseforEnglish}.
The substitutions include \{\ding{172}~idea--recommendation, \ding{173}~BUT--NEVERTHELESS, \ding{174}~It--This, \ding{175}~the--this, \ding{176}~back--end, \ding{177}~anything--whatsoever, \ding{178}~slow--obtuse, \ding{179}~I--me, \ding{180}~through--by, \ding{181}~not--n't\}.
% Every combination of pairs in the list is identified, totaling 1023 combinations.
% An adversarial example is generated for each combination by replacing all words in the combination with their synonyms.
Figures~\ref{fig:bae_adversarial_attack} and~\ref{fig:man_adversarial_attack}, with bold words representing perturbations, show LIME explanations for two predictions to adversarial examples generated by TextAttack and manually, respectively. 
All adversarial examples 
% from TextAttack 
fail to attack the model since it maintains the same prediction.
% Similarly, the manually generated example is predicted as negative with a high confidence of 0.999.
% Bold words represent perturbations in the texts.
These results indicate that although the model is robust against certain adversarial examples, its prediction can still be untrustworthy.
% We also test the potential harm of this untrustworthy prediction by synthesising two new text inputs.
% One removes all irrelevant words highlighted in orange in Figure~\ref{fig:amazon_example}, and the other is derived from a positive amazon review, shown in Figure~\ref{fig:original_trust_prediction}, with some orange-highlighted words injected into the text.
% The corresponding predictions shown in Figure~\ref{fig:amazon_remove_words} and~\ref{fig:falied_synthesised_data} are both incorrect.
% In Figure~\ref{fig:amazon_remove_words}, despite negative sentiment in phrases ``not seen him CLEAN'', ``slow'', ``rough patch'', and ``sloggin'', the model fails to predict correctly without spurious correlations.
% In Figure~\ref{fig:falied_synthesised_data}, the injected words ``back'', ``not'', and ``BUT'' are underlined and do not change the original meaning.
% However, the model fails to make a correct prediction although the original text is correctly predicted as positive with a high confidence of 0.990, as shown in Figure~\ref{fig:original_trust_prediction}.
% The model interprets the injected words as clues to predict the text as a negative review, showing that it is misled by minor spurious correlations.
% Therefore, if trustworthiness issues are not detected early, ML models cannot correctly interpret data in the real world where spurious correlations are absent, or they can be fooled by spurious correlations into making problematic predictions.

% Both predictions are incorrect, indicating that without spurious correlations, the model fails to analyse the text as negative and is also tricked when semantically meaningless spurious correlations are injected.
% These examples demonstrate the differences between trustworthiness and robustness, as well as the potential harm of individual untrustworthy predictions.

% To address the trustworthiness oracle problem effectively and efficiently, this paper proposes TOKI, an approach to generate fully automated test oracles that can assess the trustworthiness of predictions. TOKI indicates which words in the explanation are semantically related to the predicted class, thereby classifying the prediction as trustworthy or untrustworthy. This ability helps AI practitioners detect trust-related issues of the model to avoid potential harm that may occur during later usage.


% \begin{figure}[ht]
%     \centering
%     \caption{A LIME explanation of an individual prediction with a strong confidence of 0.995 made by a classifier trying to determine if a document is about ``Christianity'' or ``Atheism''. The color indicates which class the word contributes to (orange for ``Christianity'', blue for ``Atheism''). The shade represents the importance given to the most relevant words highlighted in the text.}
%     \label{fig:motivating_example}
% \end{figure}
% \begin{figure}[ht]
%     \centering
%     \caption{A LIME explanation of a prediction with a strong confidence of 0.999 made by a fine-tuned model analysing amazon polarity. The color indicates which class the word contributes to (orange for negative, blue for positive). The shade represents the importance given to the most relevant words highlighted in the text.}
%     \label{fig:motivating_example_amazon}
% \end{figure}

==> sections/slto.tex <==
This paper first introduces a supervised learning approach for automated trustworthiness oracle generation (SLTO).
A set of explanations representing predictions acts as the training dataset for SLTO. 
A crucial step in SLTO is vectorizing the explanations, as described in Figure~\ref{fig:expl_vectorization}, to input them into supervised learning. The top \textit{n} words are chosen by the explanation method. Word embeddings are then generated for the class name and the top \textit{n} words. An explanation vector is constructed by concatenating the embedding of the class name and \textit{n} word embeddings multiplied by the corresponding importance score. 
% \steven{Should define what 'importance score' is} 
% \lam{I defined ``importance score'' in Section~\ref{sec:trustworthiness_oracle_problem}}
If importance scores are not provided, each word is assigned an importance score of 1.
% If the correlation of the importance scores is not considered, each word is assigned an importance score of 1.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{figures/expl_vectorization.pdf}
    \caption{Explanation vectorization method.}
    \label{fig:expl_vectorization}
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth, clip, trim=0 0 0 2.4mm]{figures/SLTO.pdf}
    \caption{Supervised learning trustworthiness oracle using ensemble models.}
    \label{fig::ml-trust-model}
\end{figure}

\lam{Explain why we use multiples word embedding models}
Studies~\cite{Bolukbasi:2016:ManistoComputerProgrammerasWomanistoHomemakerDebiasingWordEmbeddings, Wang:2019:EvaluatingWordEmbeddingModelsMethodsAndExperimentalResults, Torregrossa:2021:ASurveyOnTrainingAndEvaluationOfWordEmbeddings, Schuster:2020:HumptyDumpty:ControllingWordMeaningsviaCorpusPoisoning} show that word embedding methods can be biased due to their training data, thereby potentially impacting their ability to generate accurate embeddings.
To address this problem, SLTO applies ensemble learning by employing \textit{k} different word embedding methods as shown in Figure~\ref{fig::ml-trust-model}.
With each word embedding method, a model is trained using trustworthiness labels and explanation vectors generated by the embedding method.
Given a new prediction and its explanation, each $model_i$ predicts a trustworthiness label \textit{trust\_label}$_i$. 
% \valerio{don't do this in latex, looks bad as there are extra space between words, do instead: \textit{trust\_label}$_i$ can you see the difference?} 
% \lam{I fixed it, thank you for showing me the right way.}
Finally, \textit{trust\_label}$_1$~--~\textit{trust\_label}$_k$ predicted by all \textit{model}$_1$~--~\textit{model}$_k$ are combined to compute the final trustworthiness label by plurality voting. 
% \valerio{It is clear to use why you are considering multiples word embedding models, but we should explain it to the reader, we need to motivate and justify key design choices like having multiple word embeddings}
% \lam{I revised this paragraph as well as the section ``Word embedding''}

==> sections/tower.tex <==
% \valerio{Since we compare with TOWER we need to move some description in the evaluation}
% \lam{I added a subsection Section~\ref{sec:expr_baselines}. ``Baselines''.}
TOWER, introduced by Cho et al.~\cite{Cho:2023:TOWER}, is the first attempt to generate automated trustworthiness oracles.
It aims to assess the trustworthiness of a correct prediction made by text classifiers using explanation methods and word embeddings. 
% % Figure~\ref{fig:tower_process} illustrates the process of TOWER.
% TOWER uses an explanation method to explain a prediction, highlighting the most relevant words.
% % Input is fed into the classifier, followed by using an explanation method to generate an explanation for it. If the classifier misclassifies, the input is disregarded by their definition of trustworthiness. 
% The relevant words are processed through a word embedding ensemble to measure their semantic relatedness to the predicted class, which is used to compute the prediction score for each prediction.
% % \begin{figure}[http]
% %     \centering
% %     \includegraphics[width=\linewidth]{figures/tower_process.png}
% %     \caption{Overall TOWER design.}
% %     \label{fig:tower_process}
% % \end{figure}
Experiments were conducted to assess how TOWER using LIME explanation method~\cite{Ribeiro:2016:WhyShouldITrustYouExplainingthePredictionsofAnyClassifier} align with the human sense of trustworthiness. 
% The selected datasets included AG news, Amazon reviews~\cite{Zhang:2015:CharacterLevelConvolutionalNetworksforTextClassification}, DBpedia 14~\cite{Lehmann:2014:DBpediaALargescaleMultilingualKnowledgeBaseExtractedfromWikipedia}, emotions~\cite{Saravia:2018:CARERContextualizedAffectRepresentationsforEmotionRecognition}, IMDb~\cite{Maas:2011:LearningWordVectorsforSentimentAnalysis}, Stanford sentiment treebank~\cite{Socher:2013:RecursiveDeepModelsforSemanticCompositionalityOveraSentimentTreebank}, Yahoo answers topics, and news groups~\cite{Ken:1995:NewsWeederLearningtoFilterNetnews}.
% The human-created ground truths consisted of 328 instances with skewed data, where 90\% of labels were deemed trustworthy. Experimental results indicate that TOWER's precision for labeling as trustworthy is 0.92, recall is 0.4, and F1 score is 0.56. For labeling as untrustworthy, these scores are 0.135, 0.476, and 0.21, respectively. 
The results reveal a bias in TOWER towards not labeling predictions as trustworthy due to the limited method of measuring trustworthiness. TOWER solely assesses how semantically related words are to the class name, which lacks accuracy and may not be meaningful enough to capture the relationship between words and classes.

==> sections/trustworthiness_vs_robustness.tex <==
With the same goal of model generalisation, trustworthiness described in Definition~\ref{def:trustworthy_prediction} and robustness
% which refers to the ability to maintain performance in uncertain or adversarial conditions~\cite{Dalvi:2004:AdversarialClassification, Biggio:2018:WildPatternsTenYearsAftertheRiseofAdversarialMachineLearning, Szegedy:2014:IntriguingPropertiesofNeuralNetworks}, 
seem similar.
Global robustness refers to the model's ability to generalise well to 
% unseen data and diverse conditions~\cite{Dalvi:2004:AdversarialClassification, Biggio:2018:WildPatternsTenYearsAftertheRiseofAdversarialMachineLearning}.
all possible data~\cite{Leino:2021:GloballyRobustNeuralNetworks}.
It is clear that global trustworthiness and global robustness overlap as the model ultimately predicts based on justifiable reasons, thereby handling unseen data effectively.
Achieving global trustworthiness and global robustness requires complex architectures and training procedures, leading to high costs~\cite{Weng:2018:TowardsFastComputationofCertifiedRobustnessforReLUNetworks}.
Consequently, existing research primarily focuses on local robustness, which is the model's ability to maintain performance despite minimal imperceptible perturbations to the inputs, also known as adversarial examples~\cite{Yuan:2019:AdversarialExamplesAttacksandDefensesforDeepLearning}.
Differ from their global counterparts, local trustworthiness and local robustness, are distinct concepts.
% % This includes handling noisy data, distribution shifts, and adversarial attacks, among other challenges.
% Although the definitions of robustness and trustworthiness described in Definition~\ref{def:trustworthy_prediction} seem similar, they are different concepts.
Given an individual instance and its prediction, trustworthiness refers to whether the prediction is mainly based on semantically related words, while robustness shows the ability to maintain performance on adversarial examples.
An intuition can be that if the model correctly predicts based on semantically unrelated words, perturbations on these words may remove the spurious correlation and make the model predict incorrectly, meaning the model is not robust on the instance. 
However, adversarial examples do not always alter the prediction since the model also learns valid correlations.
In other words, a model can be robust on the instance, but its corresponding prediction may still be untrustworthy. 

\begin{figure}[t]
    \centering
    \begin{subfigure}[ht]{0.21\linewidth}
        \centering
        \includegraphics[scale=1]{figures/trust_case1.pdf}
        \caption{}
        \label{fig:trust_case1}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[ht]{0.13\linewidth}
        \centering
        \includegraphics[scale=1]{figures/trust_case3.pdf}
        \caption{}
        \label{fig:trust_case3}
    \end{subfigure}
    \hfill
    \begin{subfigure}[ht]{0.13\linewidth}
        \centering
        \includegraphics[scale=1]{figures/trust_case2.pdf}
        \caption{}
        \label{fig:trust_case2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[ht]{0.13\linewidth}
        \centering
        \includegraphics[scale=1]{figures/trust_case4.pdf}
        \caption{}
        \label{fig:trust_case4}
    \end{subfigure}
    \hfill
    \begin{subfigure}[ht]{0.14\linewidth}
        \centering
        \includegraphics[scale=1, clip, trim=0 1.4mm 0 1.4mm]{figures/trust_case5.pdf}
        \caption{}
        \label{fig:trust_case5}
    \end{subfigure}
    \hfill
    \begin{subfigure}[ht]{0.13\linewidth}
        \centering
        \includegraphics[scale=1]{figures/trust_case6.pdf}
        \caption{}
        \label{fig:trust_case6}
    \end{subfigure}
    \caption{Different trustworthiness scenarios of a correct prediction. Circles with green, blue, and dash outlines show the desired reasoning, the original model's reasoning, and the new model's reasoning on adversarial examples, respectively.}
    \label{fig:trust_cases}
    \Description[Various trustworthiness scenarios]{Fully described in the text.}
\end{figure}

Figures~\ref{fig:trust_case1}~--~\ref{fig:trust_case6} describe various trustworthiness scenarios. 
Figure~\ref{fig:trust_case1} shows an untrustworthy prediction where the model's reasoning and the desired reasoning are completely different.
The model is not robust on the instance as its adversarial examples can easily change the prediction.
Figures~\ref{fig:trust_case2} and~\ref{fig:trust_case3} both represent trustworthy predictions where the model's reasoning mainly aligns with the desired reasoning.
Adversarial examples are unlikely to change the prediction, making the model robust on the instance.
Figure~\ref{fig:trust_case4} illustrates an untrustworthy prediction.
The model's reasoning reflects the desired reasoning but it significantly focuses on other factors.
However, adversarial examples, which maintain the original semantic meaning, do not change the model output.
The model, therefore, is robust on this instance.
Figure~\ref{fig:trust_case5} shows an untrustworthy prediction where the model's reasoning contains both a part of the desired reasoning and other factors.
In this case, the robustness of the model on the instance is hard to tell.
Adversarial examples can either change or maintain the prediction, depending on the model's behavior and the degree of overlap between the desired reasoning and the model's reasoning.
If the model's reasoning slightly reflects the desired reasoning, small perturbations can make the model predict differently.
Figure~\ref{fig:trust_case6} represents a perfectly trustworthy prediction.
The model is also robust to adversarial examples since it completely captures the true reasoning for the prediction.
These scenarios illustrate the difference between trustworthiness and robustness.
They show that although a model is robust to adversarial examples of an instance, its prediction can be untrustworthy, posing potential defects.
% In Section~\ref{sec:motivating_example}, we showcase examples to differentiate trustworthiness from robustness and the harms of untrustworthy predictions.

==> tables/naive.tex <==
\begin{table}[t]
    \caption{Comparison between TOKI and Naive with different values of $\theta$\textsubscript{\textit{conf}}}
    % \label{table:experimental_result_rq2_5_6}
    \resizebox{\linewidth}{!}{% <------ Don't forget this %
    \begin{tabular}{c|l|C|C|C|C|C|C}
        \toprule
        Dataset & \multicolumn{1}{c|}{Method}     & \multicolumn{1}{c|}{Acc}   & \multicolumn{1}{c|}{Pre}   & \multicolumn{1}{c|}{Sen}   & \multicolumn{1}{c|}{F1-score} & \multicolumn{1}{c|}{Spec}  & \multicolumn{1}{c|}{G-mean} \\
        \midrule[1pt]
        \multirow{14}{*}{\rotatebox[origin=c]{90}{Dong's~\cite{Dong:2018:ComparingAutomaticandHumanEvaluationofLocalExplanationsforTextClassification}}} & Navie-0.50                                & 0.869                        & 0.869                         & 1.000                           & 0.930                        & 0.000                           & 0.000                      \\
        & Navie-0.55                                & 0.855                        & 0.869                         & 0.981                           & 0.921                        & 0.021                           & 0.144                      \\
        & Navie-0.60                                & 0.852                        & 0.873                         & 0.971                           & 0.919                        & 0.064                           & 0.249                      \\
        & Navie-0.65                                & 0.841                        & 0.878                         & 0.949                           & 0.912                        & 0.128                           & 0.348                      \\
        & Navie-0.70                                & 0.824                        & 0.878                         & 0.926                           & 0.901                        & 0.149                           & 0.371                      \\
        & Navie-0.75                                & 0.804                        & 0.878                         & 0.900                           & 0.889                        & 0.170                           & 0.391                      \\
        & Navie-0.80                                & 0.796                        & 0.881                         & 0.884                           & 0.883                        & 0.213                           & 0.434                      \\
        & Navie-0.85                                & 0.785                        & 0.880                         & 0.871                           & 0.876                        & 0.213                           & 0.431                      \\
        & Navie-0.90                                & 0.771                        & 0.893                         & 0.836                           & 0.864                        & 0.340                           & 0.533                      \\
        & Navie-0.95                                & 0.737                        & 0.897                         & 0.788                           & 0.839                        & 0.404                           & 0.564                      \\
        % & Navie-1.00                                & 0.142                        & 1.000                         & 0.013                           & 0.025                        & 1.000                           & 0.113                      \\
        \cmidrule{2-8}
        & TOKI-lime                & 0.930                        & 0.947                         & 0.974                           & 0.960                        & 0.638                           & 0.789                      \\
        & TOKI-omis         & 0.882                        & 0.912                         & 0.956                           & 0.934                        & 0.392                           & 0.612                      \\
        & TOKI-sali        & 0.853                        & 0.944                         & 0.891                           & 0.917                        & 0.387                           & 0.587                      \\
        \midrule[1pt] 
        \multirow{12}{*}{\rotatebox[origin=c]{90}{Cho's~\cite{Cho:2023:TOWER}}} & Navie-0.50                                & 0.918                        & 0.922                         & 0.996                           & 0.957                        & 0.000                           & 0.000                      \\
        & Navie-0.55                                & 0.914                        & 0.922                         & 0.991                           & 0.955                        & 0.000                           & 0.000                      \\
        & Navie-0.60                                & 0.910                        & 0.921                         & 0.987                           & 0.953                        & 0.000                           & 0.000                      \\
        & Navie-0.65                                & 0.910                        & 0.921                         & 0.987                           & 0.953                        & 0.000                           & 0.000                      \\
        & Navie-0.70                                & 0.906                        & 0.925                         & 0.978                           & 0.951                        & 0.053                           & 0.227                      \\
        & Navie-0.75                                & 0.894                        & 0.924                         & 0.965                           & 0.944                        & 0.053                           & 0.225                      \\
        & Navie-0.80                                & 0.886                        & 0.923                         & 0.956                           & 0.939                        & 0.053                           & 0.224                      \\
        & Navie-0.85                                & 0.865                        & 0.921                         & 0.934                           & 0.927                        & 0.053                           & 0.222                      \\
        & Navie-0.90                                & 0.861                        & 0.925                         & 0.925                           & 0.925                        & 0.105                           & 0.312                      \\
        & Navie-0.95                                & 0.816                        & 0.921                         & 0.876                           & 0.898                        & 0.105                           & 0.304                      \\
        % & Navie-1.00                                & 0.078                        & 0.000                         & 0.000                           & 0.000                        & 1.000                           & 0.000                      \\
        \cmidrule{2-8}
        & TOKI-lime           & 0.922                        & 0.977                         & 0.938                           & 0.957                        & 0.737   & 0.831    \\ 
        \bottomrule
    \end{tabular}% <------ Don't forget this %
}
\end{table}


==> tables/new_example.tex <==
\begin{table}[t]
    \resizebox{\textwidth}{!}{% <------ Don't forget this %
    \begin{tabular}{p{\textwidth}c}
    Example & Prediction Probability \\
    \small Sounds like a great idea, BUT.......
    It read on the back like a great book. Inside though is another story. I am halfway thru it and I have not seen him CLEAN anything. It is too slow, but I want to still read to find out what happens.It is a rough patch now but I am sloggin through. If it does not pick up soon I will give up. Welty69        
    &                        \\
    \small Sounds like a great idea, BUT.......
    It read on the back like a great book. Inside though is another story. I am halfway thru it and I have not seen him CLEAN anything. It is too slow, but I want to still read to find out what happens.It is a rough patch now but I am sloggin through. If it does not pick up soon I will give up. Welty69        
    &                        \\
    \small Sounds like a great idea, BUT.......
    It read on the back like a great book. Inside though is another story. I am halfway thru it and I have not seen him CLEAN anything. It is too slow, but I want to still read to find out what happens.It is a rough patch now but I am sloggin through. If it does not pick up soon I will give up. Welty69        
    &                        \\
    \small Sounds like a great idea, BUT.......
    It read on the back like a great book. Inside though is another story. I am halfway thru it and I have not seen him CLEAN anything. It is too slow, but I want to still read to find out what happens.It is a rough patch now but I am sloggin through. If it does not pick up soon I will give up. Welty69        
    &                      \\
    \small Sounds like a great idea, BUT.......
    It read on the back like a great book. Inside though is another story. I am halfway thru it and I have not seen him CLEAN anything. It is too slow, but I want to still read to find out what happens.It is a rough patch now but I am sloggin through. If it does not pick up soon I will give up. Welty69        
    &                      \\
    \small Sounds like a great idea, BUT.......
    It read on the back like a great book. Inside though is another story. I am halfway thru it and I have not seen him CLEAN anything. It is too slow, but I want to still read to find out what happens.It is a rough patch now but I am sloggin through. If it does not pick up soon I will give up. Welty69        
    &                      \\
    \end{tabular}%
    }
\end{table}


==> tables/slto_comparison.tex <==
\begin{table*}[ht]
    \caption{Comparison between SLTO, TOKI and the benchmarks with different explanation methods against the split test set}
    \label{table:experimental_result_rq5}\resizebox{0.981\textwidth}{!}{% <------ Don't forget this %
    \begin{tabular}{l|l|C|C|C|C|C|C|c|c|c|c}
        \toprule
        Dataset & Method & \multicolumn{1}{c|}{Acc}   & \multicolumn{1}{c|}{Pre}   & \multicolumn{1}{c|}{Sen}   & \multicolumn{1}{c|}{F1-score} & \multicolumn{1}{c|}{Spec}  & \multicolumn{1}{c|}{G-mean} & \makecell{Training\\Instances} & \makecell{Training\\Time (s)}  & \makecell{Test\\Instances}      & \makecell{Evaluation\\Time (s)} \\
        \midrule[1pt]
        % \multicolumn{11}{c}{movie dataset}                                                                                                \\
        % \midrule
        \multirow{10}{0.6cm}{movie dataset}  & TOKI-lime     & 0.814 & 0.800 & 1.000 & 0.889 & 0.600 & 0.775 & \multirow{3}{1.6cm}{1,430 (w/o trustworthiness labels)} & \multirow{3}{*}{\xmark} & \multirow{10}{*}{43} & 240       \\
                                            & TOKI-omis     & 0.930 & 0.975 & 0.951 & 0.963 & 0.500 & 0.670 &  &  &                     & 127       \\
                                            & TOKI-sali     & 0.791 & 0.914 & 0.842 & 0.877 & 0.500 & 0.649 & &  &                     & 181       \\
        \cmidrule{2-10}
        \cmidrule{12-12}
                                            & SLTO-lime     & 0.721 & 0.897 & 0.814 & 0.852 & 0.200 & 0.403 & \multirow{3}{1.6cm}{157 (w/ trustworthiness labels)} & 494    &                     & 259       \\
                                            & SLTO-omis     & 0.767 & 1.000 & 0.780 & 0.877 & 0.500 & 0.625 &     & 69     &                     & 73        \\
                                            & SLTO-sali     & 0.884 & 0.884 & 1.000 & 0.938 & 0.000 & 0.000 &     & 55     &                     & 157       \\
        \cmidrule{2-10}
        \cmidrule{12-12}
        % \cmidrule{2-10}
        % \cmidrule{12-12}
                                            & Naive         & 0.629 & 0.758 & 0.781 & 0.769 & 0.400 & 0.559 & \xmark                           & \xmark &                     & \xmark    \\
        \cmidrule{2-10}
        \cmidrule{12-12}
                                            & TOWER-lime    & 0.349 & 0.800 & 0.375 & 0.511 & 0.600 & 0.474 & \multirow{3}{*}{\xmark}                & \multirow{3}{*}{\xmark} &                     & 232     \\
                                            & TOWER-omis    & 0.279 & 1.000 & 0.244 & 0.392 & 1.000 & 0.494 &                            &  &                     & 118    \\
                                            & TOWER-sali    & 0.302 & 1.000 & 0.263 & 0.417 & 0.750 & 0.444 &                            &  &                     & 179    \\
        \midrule[1pt]
        \multirow{10}{0.6cm}{20news dataset} & TOKI-lime     & 0.810 & 0.795 & 1.000 & 0.886 & 0.429 & 0.655 & \multirow{3}{1.6cm}{1,079 (w/o trustworthiness labels)} & \multirow{3}{*}{\xmark} & \multirow{10}{*}{42} & 214       \\
                                            & TOKI-omis     & 0.857 & 0.875 & 0.972 & 0.921 & 0.200 & 0.441 &   & &                     & 145       \\
                                            & TOKI-sali     & 0.905 & 0.902 & 1.000 & 0.949 & 0.250 & 0.500 &   &  &                     & 194       \\
        \cmidrule{2-10}
        \cmidrule{12-12}
                                            & SLTO-lime     & 0.381 & 0.818 & 0.290 & 0.429 & 0.857 & 0.499 & \multirow{3}{1.6cm}{155 (w/ trustworthiness labels)} & 422    &                     & 268       \\
                                            & SLTO-omis     & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 &     & 76     &                     & 106       \\
                                            & SLTO-sali     & 0.690 & 0.903 & 0.757 & 0.824 & 0.000 & 0.000 &     & 71     &                     & 178       \\
        \cmidrule{2-10}
        \cmidrule{12-12}
        % \cmidrule{2-10}
        % \cmidrule{12-12}
                                            & Naive         & 0.690 & 0.757 & 0.903 & 0.825 & 0.143 & 0.359 & \xmark                           & \xmark &                     & \xmark    \\
        \cmidrule{2-10}
        \cmidrule{12-12}
                                            & TOWER-lime    & 0.214 & 1.000 & 0.065 & 0.121 & 1.000 & 0.254 & \multirow{3}{*}{\xmark}                           & \multirow{3}{*}{\xmark} &                     & 205    \\
                                            & TOWER-omis    & 0.167 & 1.000 & 0.056 & 0.105 & 1.000 & 0.236 &                            &  &                     & 136    \\
                                            & TOWER-sali    & 0.095 & --     & 0.000 & 0.000 & 0.750 & 0.000 &                            &  &                     & 187    \\
        \bottomrule
    \end{tabular}% <------ Don't forget this %
}
\end{table*}

==> tables/slto_merge.tex <==
\begin{table*}[ht]
    \caption{Comparison between SLTO, TOKI and the benchmarks with different explanation methods against the split test set}
    \label{table:experimental_result_rq5}
    % \resizebox{0.981\textwidth}{!}{% <------ Don't forget this %
    \begin{tabular}{l|l|C|C|C|C|C|C|c|c|c|c}
        \toprule
        Dataset & Method & \multicolumn{1}{c|}{Acc}   & \multicolumn{1}{c|}{Pre}   & \multicolumn{1}{c|}{Sen}   & \multicolumn{1}{c|}{F1-score} & \multicolumn{1}{c|}{Spec}  & \multicolumn{1}{c|}{G-mean} & \makecell{Training\\Instances} & \makecell{Training\\Time (s)}  & \makecell{Test\\Instances}      & \makecell{Evaluation\\Time (s)} \\
        \midrule[1pt]
        % \multicolumn{11}{c}{movie dataset}                                                                                                \\
        % \midrule
        \multirow{10}{*}{Dong's}  & TOKI-lime     & 0.812 & 0.797 & 1.000 & 0.887 & 0.666 & 0.707 & \multirow{3}{1.6cm}{2,509 (w/o trustworthiness labels)} & \multirow{3}{*}{\xmark} & \multirow{10}{*}{85} & 454       \\
                                            & TOKI-omis     & 0.894 & 0.925 & 0.961 & 0.943 & 0.286 & 0.524 &  &  &                     & 272       \\
                                            & TOKI-sali     & 0.847 & 0.908 & 0.920 & 0.914 & 0.375 & 0.587 & &  &                     & 375       \\
        \cmidrule{2-10}
        \cmidrule{12-12}
                                            & SLTO-lime     & 0.553 & 0.875 & 0.556 & 0.680 & 0.583 & 0.569 & \multirow{3}{1.6cm}{312 (w/ trustworthiness labels)} & 916    &                     & 427       \\
                                            & SLTO-omis     & 0.388 & 0.941 & 0.416 & 0.577 & 0.143 & 0.244 &     & 145     &                     & 179        \\
                                            & SLTO-sali     & 0.788 & 0.892 & 0.880 & 0.886 & 0.000 & 0.000 &     & 126     &                     & 335       \\
        \cmidrule{2-10}
        \cmidrule{12-12}
        % \cmidrule{2-10}
        % \cmidrule{12-12}
                                            & Naive         & 0.659 & 0.757 & 0.841 & 0.797 & 0.250 & 0.459 & \xmark                           & \xmark &                     & \xmark    \\
        \cmidrule{2-10}
        \cmidrule{12-12}
                                            & TOWER-lime    & 0.282 & 0.824 & 0.222 & 0.350 & 0.833 & 0.430 & \multirow{3}{*}{\xmark}                & \multirow{3}{*}{\xmark} &                     & 437     \\
                                            & TOWER-omis    & 0.224 & 1.000 & 0.156 & 0.270 & 1.000 & 0.395 &                            &  &                     & 254    \\
                                            & TOWER-sali    & 0.200 & 1.000 & 0.133 & 0.235 & 0.750 & 0.316 &                            &  &                     & 366    \\
        \bottomrule
    \end{tabular}% <------ Don't forget this %
% }
\end{table*}

==> tables/toki_comparison.tex <==
\begin{table*}[ht]
    \caption{Comparison between TOKI and the benchmarks with different explanation methods against the ground truths}
    \label{table:experimental_result_rq2_5_6}
    \resizebox{\textwidth}{!}{% <------ Don't forget this %
    \begin{tabular}{l|l|C|C|C|C|C|C|c|c|c|c}
        \toprule
        Dataset & Method                     & \multicolumn{1}{c|}{Acc}   & \multicolumn{1}{c|}{Pre}   & \multicolumn{1}{c|}{Sen}   & \multicolumn{1}{c|}{F1-score} & \multicolumn{1}{c|}{Spec}  & \multicolumn{1}{c|}{G-mean} & \makecell{Training\\Instances} & \makecell{Keyword\\Identification\\Time (s)} & \makecell{Test\\Instances} & \makecell{Evaluation\\Time (s)} \\
        \midrule[1pt]
        \multirow{7}{1.1cm}{movie dataset} & TOKI-lime                  & 0.815 & 0.849 & 0.950 & 0.897    & 0.611 & 0.762  & \multirow{3}{*}{1,430} & 3,161                        & \multirow{7}{*}{200} & 620                \\
        & TOKI-omis              & 0.890 & 0.939 & 0.939 & 0.939    & 0.450 & 0.650  &                       & 63                          &                      & 190                \\
        & TOKI-sali              & 0.795 & 0.941 & 0.786 & 0.867    & 0.563 & 0.665  &                       & 25                          &                      & 339                \\
        \cmidrule{2-10}
        \cmidrule{12-12}
        & Naive                      & 0.710 & 0.829 & 0.850 & 0.840    & 0.333 & 0.532  & \xmark                & \xmark                      &                      & \xmark             \\
        \cmidrule{2-10}
        \cmidrule{12-12}
        & TOWER-lime                      & 0.385 & 0.875 & 0.394 & 0.543    & 0.667 & 0.512  & \multirow{3}{*}{\xmark}                & \multirow{3}{*}{\xmark}                      &                      & 613                \\
        & TOWER-omis                      & 0.360 & 0.967 & 0.322 & 0.483    & 0.700 & 0.475  &                 &                       &                      & 178                \\
        & TOWER-sali                      & 0.340 & 0.982 & 0.302 & 0.462    & 0.813 & 0.396  &                 &                       &                      & 331                \\
        \midrule[1pt]
        \multirow{7}{1.1cm}{20news dataset} & TOKI-lime                  & 0.863 & 0.848 & 1.000 & 0.918    & 0.655 & 0.809  & \multirow{3}{*}{1,079} & 1,705                        & \multirow{7}{*}{197} & 540                \\
        & TOKI-omis              & 0.838 & 0.846 & 0.975 & 0.906    & 0.355 & 0.588  &                       & 35                          &                      & 223                \\
        & TOKI-sali              & 0.918 & 0.918 & 1.000 & 0.957    & 0.200 & 0.447  &                       & 16                          &                      & 427                \\
        \cmidrule{2-10}
        \cmidrule{12-12}
        & Naive                      & 0.726 & 0.781 & 0.921 & 0.845    & 0.138 & 0.356  & \xmark                & \xmark                      &                      & \xmark             \\
        \cmidrule{2-10}
        \cmidrule{12-12}
        & TOWER-lime                      & 0.239 & 1.000 & 0.119 & 0.213    & 1.000 & 0.345  & \multirow{3}{*}{\xmark}                & \multirow{3}{*}{\xmark}                      &                      & 536                \\
        & TOWER-omis                      & 0.254 & 1.000 & 0.127 & 0.225    & 0.968 & 0.225  &                 &                       &                      & 218                \\
        & TOWER-sali                      & 0.051 & -     & 0.000 & 0.000    & 0.600 & 0.000  &                 &                       &                      & 421                \\
        \midrule[1pt]
        \multirow{3}{1.1cm}{ag\_news dataset} & TOKI-lime                  & 0.935 & 0.952 & 0.976 & 0.964    & 1.000 & 0.988  & 2,000                  & 34,532                       & \multirow{3}{*}{46}  & 1,148                \\
        \cmidrule{2-10}
        \cmidrule{12-12}
        & Naive                      & 0.870 & 0.889 & 0.976 & 0.930    & 0.000 & 0.000  & \xmark                & \xmark                      &                      & \xmark             \\
        \cmidrule{2-10}
        \cmidrule{12-12}
        & TOWER-lime                      & 0.304 & 0.917 & 0.268 & 0.415    & 1.000 & 0.518  & \xmark                & \xmark                      &                      & 1,072               \\
        \midrule[1pt]
        \multirow{3}{1.1cm}{amazon dataset} & TOKI-lime                  & 0.882 & 0.891 & 0.976 & 0.932    & 0.571 & 0.747  & 2,000                  & 488,791                      & \multirow{3}{*}{51}  & 12,654                \\
        \cmidrule{2-10}
        \cmidrule{12-12}
        & Naive                      & 0.824 & 0.824 & 1.000 & 0.903    & 0.000 & 0.000  & \xmark                & \xmark                      &                      & \xmark             \\
        \cmidrule{2-10}
        \cmidrule{12-12}
        & TOWER-lime                      & 0.333 & 0.875 & 0.333 & 0.483    & 0.286 & 0.309  & \xmark                & \xmark                      &                      & 12,637                \\
        \bottomrule
    \end{tabular}% <------ Don't forget this %
}
\end{table*}


==> tables/toki_f1.tex <==
\begin{table*}[ht]
    \caption{Comparison between TOKI and the benchmarks with different explanation methods against the ground truths}
    \label{table:experimental_result_rq2_5_6}
    \resizebox{\textwidth}{!}{% <------ Don't forget this %
    \begin{tabular}{c|l|C|C|C|C|C|c|c|c|c}
        \toprule
        Dataset & \multicolumn{1}{c|}{Method}     & \multicolumn{1}{c|}{Acc}   & \multicolumn{1}{c|}{F1-tru}   & \multicolumn{1}{c|}{F1-unt}   & \multicolumn{1}{c|}{F1-bal} & \multicolumn{1}{c|}{AUCROC}  & \makecell{\small Training\\Instances} & \makecell{\small Keyword\\Identification\\Time (s)} & \makecell{\small Test\\Instances} & \makecell{\small Trustworthiness\\Label Computa-\\tion Time (s)} \\
        \midrule[1pt]
        \multirow{3}{*}{\rotatebox[origin=c]{90}{\makecell{CAMS\\\cite{Garg:2022:CAMS:AnAnnotatedCorpusforCausalAnalysisofMentalHealthIssuesinSocialMediaPosts}}}} & TOKI-lime                  & 0.878 & 0.905 & 0.829 & 0.866    &  0.882  & \multirow{1}{*}{2,158} & 198,359                        & \multirow{3}{*}{1,945} & 224,540                \\
        \cmidrule{2-9}
        \cmidrule{11-11}
         & Naive                      & 0.592 & 0.789 & 0.466 & 0.586    & 0.797 & 0.609  & \xmark                & \xmark                      &                      & \xmark             \\
        \cmidrule{2-10}
        \cmidrule{12-12}
         & TOKI-lime$^\ominus$                      & 0.422 & 0.648 & 0.343 & 0.449    & 0.551 & 0.435  & \xmark                & \xmark                      &                      & 224,528             \\
        \midrule[1pt]
        \multirow{7}{*}{\rotatebox[origin=c]{90}{Dong's~\cite{Dong:2018:ComparingAutomaticandHumanEvaluationofLocalExplanationsforTextClassification}}} & TOKI-lime                  & 0.930 & 0.947 & 0.974 & 0.960    & 0.638 & 0.789  & \multirow{3}{*}{2,509} & 4,866                        & \multirow{7}{*}{358} & 1,053                \\
        & TOKI-omis              & 0.882 & 0.912 & 0.956 & 0.934    & 0.392 & 0.612  &                       & 98                          &                      & 379                \\
        & TOKI-sali              & 0.853 & 0.944 & 0.891 & 0.917    & 0.387 & 0.587  &                       & 41                          &                      & 704                \\
        \cmidrule{2-10}
        \cmidrule{12-12}
        % & Naive                      & 0.796 & 0.881 & 0.884 & 0.884    & 0.213 & 0.434  & \xmark                & \xmark                      &                      & \xmark             \\
        & Naive                      & 0.737 & 0.897 & 0.788 & 0.839    & 0.404 & 0.564  & \xmark                & \xmark                      &                      & \xmark             \\
        \cmidrule{2-10}
        \cmidrule{12-12}
        & TOKI-lime$^\ominus$            & 0.302 & 0.985 & 0.209 & 0.345    & 0.915 & 0.437  & \multirow{3}{*}{\xmark}                & \multirow{3}{*}{\xmark}                      &                      & 1,041                \\
        & TOKI-omis$^\ominus$                & 0.285 & 0.956 & 0.192 & 0.320    & 0.902 & 0.416  &                 &                       &                      & 356                \\
        & TOKI-sali$^\ominus$               & 0.233 & 1.000 & 0.170 & 0.290    & 0.968 & 0.406  &                 &                       &                      & 732                \\
        \midrule[1pt]
        \multirow{3}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.4cm}{\centering Ours}}} & TOKI-lime                  & 0.922 & 0.977 & 0.938 & 0.957    & 0.737 & 0.831  & 12,000                  & 1,126,453                       & \multirow{3}{*}{245}  &  23,892  \\
        \cmidrule{2-10}
        \cmidrule{12-12}
        & Naive                      & 0.816 & 0.921 & 0.876 & 0.898    & 0.105 & 0.304  & \xmark                & \xmark                      &                      & \xmark             \\
        % & Naive                      & 0.886 & 0.923 & 0.956 & 0.939    & 0.053 & 0.224  & \xmark                & \xmark                      &                      & \xmark             \\
        \cmidrule{2-10}
        \cmidrule{12-12}
        & TOKI-lime$^\ominus$                 & 0.408 & 0.968 & 0.403 & 0.569    & 0.474 & 0.437  & \xmark                & \xmark                      &                      &  23,867              \\
        \bottomrule
    \end{tabular}% <------ Don't forget this %
}
\end{table*}


==> tables/toki_merge.tex <==
\begin{table*}[ht]
    \caption{Comparison between TOKI and the benchmarks with different explanation methods against the ground truths}
    \label{table:experimental_result_rq2_5_6}
    \resizebox{\textwidth}{!}{% <------ Don't forget this %
    \begin{tabular}{c|l|C|C|C|C|C|C|c|c|c|c}
        \toprule
        Dataset & \multicolumn{1}{c|}{Method}     & \multicolumn{1}{c|}{Acc}   & \multicolumn{1}{c|}{Pre}   & \multicolumn{1}{c|}{Sen}   & \multicolumn{1}{c|}{F1-score} & \multicolumn{1}{c|}{Spec}  & \multicolumn{1}{c|}{G-mean} & \makecell{Training\\Instances} & \makecell{Keyword\\Identification\\Time (s)} & \makecell{Test\\Instances} & \makecell{Trustworthiness\\Label Computa-\\tion Time (s)} \\
        \midrule[1pt]
        \multirow{7}{*}{Dong's} & TOKI-lime                  & 0.839 & 0.849 & 0.974 & 0.907    & 0.638 & 0.789  & \multirow{3}{*}{2,509} & 4,866                        & \multirow{7}{*}{397} & 1,160                \\
        & TOKI-omis              & 0.864 & 0.892 & 0.956 & 0.923    & 0.392 & 0.612  &                       & 98                          &                      & 413                \\
        & TOKI-sali              & 0.838 & 0.928 & 0.891 & 0.909    & 0.387 & 0.587  &                       & 41                          &                      & 730                \\
        \cmidrule{2-10}
        \cmidrule{12-12}
        & Naive                      & 0.718 & 0.804 & 0.884 & 0.842    & 0.213 & 0.434  & \xmark                & \xmark                      &                      & \xmark             \\
        \cmidrule{2-10}
        \cmidrule{12-12}
        & TOWER-lime                      & 0.312 & 0.900 & 0.260 & 0.404    & 0.872 & 0.477  & \multirow{3}{*}{\xmark}                & \multirow{3}{*}{\xmark}                      &                      & 1,149                \\
        & TOWER-omis                      & 0.307 & 0.975 & 0.231 & 0.373    & 0.863 & 0.446  &                 &                       &                      & 396                \\
        & TOWER-sali                      & 0.197 & 0.982 & 0.153 & 0.265    & 0.710 & 0.330  &                 &                       &                      & 752                \\
        \midrule[1pt]
        \multirow{4}{6mm}{Cho et al.'s} & TOKI-lime                  & 0.872 & 0.926 & 0.938 & 0.931    & 0.737 & 0.831  & 12,000                  & 1,126,453                       & \multirow{3}{*}{259}  &  24,224  \\
        \cmidrule{2-10}
        \cmidrule{12-12}
        & Naive                      & 0.838 & 0.874 & 0.956 & 0.913    & 0.053 & 0.224  & \xmark                & \xmark                      &                      & \xmark             \\
        \cmidrule{2-10}
        \cmidrule{12-12}
        & TOWER-lime                      & 0.397 & 0.901 & 0.403 & 0.557    & 0.474 & 0.437  & \xmark                & \xmark                      &                      &  24,187              \\
        \bottomrule
    \end{tabular}% <------ Don't forget this %
}
\end{table*}


==> tables/toki_new_naive.tex <==
\begin{table*}[ht]
    \caption{Comparison between TOKI and the benchmarks with different explanation methods against the ground truths}
    \label{table:experimental_result_rq2_5_6}
    \resizebox{\textwidth}{!}{% <------ Don't forget this %
    \begin{tabular}{c|l|C|C|C|C|C|C|c|c|c|c}
        \toprule
        Dataset & \multicolumn{1}{c|}{Method}     & \multicolumn{1}{c|}{Acc}   & \multicolumn{1}{c|}{Pre}   & \multicolumn{1}{c|}{Sen}   & \multicolumn{1}{c|}{F1-score} & \multicolumn{1}{c|}{Spec}  & \multicolumn{1}{c|}{G-mean} & \makecell{Training\\Instances} & \makecell{Keyword\\Identification\\Time (s)} & \makecell{Test\\Instances} & \makecell{Trustworthiness\\Label Computa-\\tion Time (s)} \\
        \midrule[1pt]
        \multirow{7}{*}{\rotatebox[origin=c]{90}{Dong's~\cite{Dong:2018:ComparingAutomaticandHumanEvaluationofLocalExplanationsforTextClassification}}} & TOKI-lime                  & 0.930 & 0.947 & 0.974 & 0.960    & 0.638 & 0.789  & \multirow{3}{*}{2,509} & 4,866                        & \multirow{7}{*}{358} & 1,053                \\
        & TOKI-omis              & 0.882 & 0.912 & 0.956 & 0.934    & 0.392 & 0.612  &                       & 98                          &                      & 379                \\
        & TOKI-sali              & 0.853 & 0.944 & 0.891 & 0.917    & 0.387 & 0.587  &                       & 41                          &                      & 704                \\
        \cmidrule{2-10}
        \cmidrule{12-12}
        & Naive                      & 0.612 & 0.948 & 0.585 & 0.724    & 0.787 & 0.679  & \xmark                & \xmark                      &                      & \xmark             \\
        \cmidrule{2-10}
        \cmidrule{12-12}
        & TOWER-lime                      & 0.302 & 0.985 & 0.209 & 0.345    & 0.915 & 0.437  & \multirow{3}{*}{\xmark}                & \multirow{3}{*}{\xmark}                      &                      & 1,041                \\
        & TOWER-omis                      & 0.285 & 0.956 & 0.192 & 0.320    & 0.902 & 0.416  &                 &                       &                      & 356                \\
        & TOWER-sali                      & 0.233 & 1.000 & 0.170 & 0.290    & 0.968 & 0.406  &                 &                       &                      & 732                \\
        \midrule[1pt]
        \multirow{3}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.4cm}{\centering Cho et al.'s~\cite{Cho:2023:TOWER}}}} & TOKI-lime                  & 0.922 & 0.977 & 0.938 & 0.957    & 0.737 & 0.831  & 12,000                  & 1,126,453                       & \multirow{3}{*}{245}  &  23,892  \\
        \cmidrule{2-10}
        \cmidrule{12-12}
        & Naive                      & 0.571 & 0.912 & 0.593 & 0.718    & 0.316 & 0.433  & \xmark                & \xmark                      &                      & \xmark             \\
        \cmidrule{2-10}
        \cmidrule{12-12}
        & TOWER-lime                      & 0.408 & 0.968 & 0.403 & 0.569    & 0.474 & 0.437  & \xmark                & \xmark                      &                      &  23,867              \\
        \bottomrule
    \end{tabular}% <------ Don't forget this %
}
\end{table*}


==> tables/toki_shorten.tex <==
\begin{table*}[ht]
    \caption{Comparison between TOKI and the benchmarks with different explanation methods against the ground truths}
    \label{table:experimental_result_rq2_5_6}
    \resizebox{\textwidth}{!}{% <------ Don't forget this %
    \begin{tabular}{c|l|C|C|C|C|c|c|c|c}
        \toprule
        Dataset & \multicolumn{1}{c|}{Method}     & \multicolumn{1}{c|}{Acc}   & \multicolumn{1}{c|}{F1-trust} & \multicolumn{1}{c|}{F1-untru} & \multicolumn{1}{c|}{G-mean} & \makecell{Training\\Instances} & \makecell{Keyword\\Identification\\Time (s)} & \makecell{Test\\Instances} & \makecell{Trustworthiness\\Label Computa-\\tion Time (s)} \\
        \midrule[1pt]
        \multirow{7}{*}{\rotatebox[origin=c]{90}{Dong's~\cite{Dong:2018:ComparingAutomaticandHumanEvaluationofLocalExplanationsforTextClassification}}} & TOKI-lime                  & 0.930 & 0.960    & 0.706   &  0.789  & \multirow{3}{*}{2,509} & 4,866                        & \multirow{7}{*}{358} & 1,053                \\
        & TOKI-omis              & 0.882 & 0.934    & 0.465 & 0.612  &                       & 98                          &                      & 379                \\
        & TOKI-sali              & 0.853 & 0.917    & 0.296  &  0.587 &                    & 41                          &                      & 704                \\
        \cmidrule{2-8}
        \cmidrule{10-10}
        & Naive                      & 0.796 & 0.883    & 0.215 & 0.434 & \xmark                & \xmark                      &                      & \xmark             \\
        \cmidrule{2-8}
        \cmidrule{10-10}
        & TOWER-lime                      & 0.302 & 0.345    & 0.295 & 0.437 & \multirow{3}{*}{\xmark}                & \multirow{3}{*}{\xmark}                      &                      & 1,041                \\
        & TOWER-omis                      & 0.285 & 0.320    & 0.285  & 0.416 &                &                       &                      & 356                \\
        & TOWER-sali                      & 0.233 & 0.290    & 0.190  &  0.406 &            &                       &                      & 732                \\
        \midrule[1pt]
        \multirow{3}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1.4cm}{\centering Cho et al.'s~\cite{Cho:2023:TOWER}}}} & TOKI-lime                  & 0.931 & 0.961    & 0.653 & 0.831 & 12,000                  & 1,126,453                       & \multirow{3}{*}{245}  &  23,892  \\
        \cmidrule{2-8}
        \cmidrule{10-10}
        & Naive                      & 0.886 & 0.939    & 0.067 & 0.224 & \xmark                & \xmark                      &                      & \xmark             \\
        \cmidrule{2-8}
        \cmidrule{10-10}
        & TOWER-lime                      & 0.408 & 0.569    & 0.234  & 0.437 & \xmark                & \xmark                      &                      &  23,867              \\
        \bottomrule
    \end{tabular}% <------ Don't forget this %
}
\end{table*}

